Extensible Proxy for Efficient NAS

Neural Architecture Search (NAS) has become a de facto approach in the recent trend of AutoML to design deep neural networks (DNNs). Efficient or near-zero-cost NAS proxies are further proposed to address the demanding computational issues of NAS, where each candidate architecture network only requires one iteration of backpropagation. The values obtained from the proxies are considered the predictions of architecture performance on downstream tasks. However, two significant drawbacks hinder the extended usage of Efficient NAS proxies. (1) Efficient proxies are not adaptive to various search spaces. (2) Efficient proxies are not extensible to multi-modality downstream tasks. Based on the observations, we design a Extensible proxy (Eproxy) that utilizes self-supervised, few-shot training (i.e., 10 iterations of backpropagation) which yields near-zero costs. The key component that makes Eproxy efficient is an untrainable convolution layer termed barrier layer that add the non-linearities to the optimization spaces so that the Eproxy can discriminate the performance of architectures in the early stage. Furthermore, to make Eproxy adaptive to different downstream tasks/search spaces, we propose a Discrete Proxy Search (DPS) to find the optimized training settings for Eproxy with only handful of benchmarked architectures on the target tasks. Our extensive experiments confirm the effectiveness of both Eproxy and Eproxy+DPS. Code is available at https://github.com/leeyeehoo/GenNAS-Zero.

==> related_work.tex <==
% Related Works
\section{Related Work}

\subsection{evolutionary NAS}
% AmoebaNet: https://arxiv.org/abs/1802.01548
AmoebaNet adopts a regularised evolutionary algorithm called Aging Evolution.

\subsection{predictor-assisted NAS}
Predictor-assisted NAS methods train predictors of the models' performance based on their topology structures.
% PNAS: https://arxiv.org/abs/1712.00559
PNAS adopts a sequential model-based optimisation (SMBO) search algorithm and a multi-layer perceptron (MLP) ensemble predictor.
% WeakNAS: https://arxiv.org/pdf/2102.10490.pdf
WeakNAS guided by the previously learned predictor and estimate a new better weak predictor
% NAO https://arxiv.org/abs/1808.07233
NAO project the topology of network architectures to a continuous space.

\subsection{zero-cost NAS}
Zero-cost NAS methods adopt measurements that can be derived efficiently to indicate the performance of the model instead of its accuracy on target task to avoid training cost. Some criterion used to be use in pruning task are used as performance indicators when performing NAS.
% SNIP: https://arxiv.org/abs/1810.02340
SNIP a saliency criterion based on connection sensitivity that identifies structurally important connections in the network for the given task. % GraPS: https://arxiv.org/abs/2002.07376
GraPS is a pruning criterion improved on the snip metric by approximating the change in gradient norm.
% synflow: https://arxiv.org/abs/2006.05467
Synflow is modified version which modified from previous synaptic saliency criterions which avoids layer collapse when performing parameter pruning.
% fisher: https://arxiv.org/abs/1801.05787
Fisher is another criterion which first used in pruning to measure the channel with least effectiveness
% jaccob covariance NASWOT https://arxiv.org/pdf/2006.04647.pdf
NASWOT designed jac\_cov score in NAS to rank neural networks instead of using accuracy.
% tenas: https://arxiv.org/pdf/2102.11535.pdf
